A 3D benchmark problem for crack propagation in brittle fracture

We propose a full 3D benchmark problem for brittle fracture based on experiments as well as a validation in the context of phase-field models. The example consists of a series of four-point bending tests on graphite specimens with sharp V-notches at different inclination angles. This simple setup leads to a mixed mode (I + II + III) loading which results in complex yet stably reproducible crack surfaces. The proposed problem is well suited for benchmarking numerical methods for brittle fracture and allows for a quantitative comparison of failure loads and propagation paths as well as initiation angles and the fracture surface. For evaluation of the crack surfaces image-based 3D models of the fractured specimen are provided along with experimental and numerical results. In addition, measured failure loads and computed load-displacement curves are given. To demonstrate the applicability of the benchmark problem, we show that for a phase-field model based on the Finite Cell Method and multi-level hp-refinement the complex crack surface as well as the failure loads can be well reproduced.

==> general/acknowledgements.tex <==
The first and the last author gratefully acknowledge the
financial support of the German Research Foundation (DFG) under
Grant RA 624/xx-1. The support of the German Israelian Foundation ....  \todo{grant eintragen}.



==> general/commonCommands.tex <==
\newcommand{\hpd}[0]{\mbox{$hp$-$d$}\xspace}

\newcommand{\refSection}[1]{Section~\ref{#1}}
\newcommand{\refFigure}[1]{Figure~\ref{#1}}
\newcommand{\refTable}[1]{Table~\ref{#1}}
\newcommand{\refEquation}[1]{(\ref{#1})}

\newcommand{\redPart}[1]{\color{red}#1\color{black}}

\newcommand{\etal}{~\textit{et al.}\xspace}

\newcommand{\tensor}[1]{\boldsymbol{{#1}}}
\newcommand{\trans}{^{\top}}
\newcommand{\integral}[3]{\int\limits_{#1} #2 \, \mathrm{d}#3}

\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcolumntype{L}[1]{>{\raggedleft\arraybackslash}m{#1}}


% \newcommand{\revOne}[1]{\color{red}#1\color{black}\xspace}
% \newcommand{\revTwo}[1]{\color{blue}#1\color{black}\xspace}
% \newcommand{\revBoth}[1]{\color{orange}#1\color{black}\xspace}
%  \newcommand{\delete}[1]{\sout{#1}\xspace}

\newcommand{\revOne}[1]{#1\xspace}
\newcommand{\revTwo}[1]{#1\xspace}
\newcommand{\revBoth}[1]{#1\xspace}
\newcommand{\delete}[1]{\xspace}

%\newcommand{\delete}[1]{}

\newcommand{\figFilename}{test.png}

\newcommand{\includeTikzFile}[3]{
  file = #1\\
  width = #2

  \renewcommand{\figFilename}{#1}
  \tikzpicturedependsonfile{\figFilename.tikz}
  \tikzsetnextfilename{\figFilename}
  \includegraphics[width = #2, 
                   height = #3]
                   {\figFilename.tikz}%
}

\newcommand{\wbalTwo}[2] {
  This is the Wikibook about LaTeX
  supported by #1 and #2}


==> general/journalFooter.tex <==
\usepackage{fancyhdr}
\date{}
\fancypagestyle{plain}{%
  \renewcommand{\headrulewidth}{0pt}%
  \fancyhf{}%
  \fancyfoot[L]{
  \vspace{-1.25cm} 
  \footnotesize{Preprint submitted to \textit{\journal{}}  \hfill
  \publicationDate
  \\
  %The final publication is available at
  % \url{http://link.springer.com/article/10.1007/s00466-014-1118-x} 
  }} }

==> general/keywords.tex <==
IGA, trimmed patches, high-order FEM, Finite Cell Method, 

==> general/packages.tex <==
\usepackage{color} 
\usepackage{psfrag} 
\usepackage{subfig}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{graphics}
 \usepackage{pstool} 
%\usepackage[on]{auto-pst-pdf}     
\usepackage{todonotes}
          
%\usepackage[square, authoryear]{natbib}
\usepackage[square,sort,comma,numbers]{natbib}
 
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{filecontents}

\usepackage{tikz}
\usepackage{tikzscale}


\usetikzlibrary{spy}
\usetikzlibrary{snakes,arrows,shapes}    
\usetikzlibrary{spy}
\usetikzlibrary{backgrounds}  
\usetikzlibrary{decorations}
\usetikzlibrary{positioning}
\usetikzlibrary{patterns}
\usetikzlibrary{calc} 
%\usetikzlibrary{external} % Is activated with the command '\tikzexternalize'.
%\tikzexternalize % To activate the externalization. 

\usepackage{booktabs}   
\usepackage{makecell} 
\usepackage{colortbl}   

\usepackage{xspace}
\usepackage{color}     
\usepackage{setspace}   
 
\usepackage{soul}
\usepackage{ulem}
\usepackage{currfile}
\usepackage{import}

\usepackage{authoraftertitle} % used for getting the authors 
\usepackage{authblk} % used for affiliations 
\renewcommand\Affilfont{\fontsize{9}{10.8}\selectfont}

\usepackage{cleveref}

==> general/pgfplotsettings.tex <==
\pgfplotsset{compat=1.8}

\newcommand{\findmax}[3]{
%     \pgfplotsforeachungrouped \table in {#1} {%
%         \pgfplotstablevertcat{\concatenated}{\table}%
%     }%
    \pgfplotstablesort[sort key={#2},sort cmp={float >}]{\sorted}{#1}%
    \pgfplotstablegetelem{0}{#2}\of{\sorted}%
    \let #3=\pgfplotsretval%
}

\pgfplotscreateplotcyclelist{myCycleListBlackAndWhite}
{%
  {black, mark=o},
  {black, mark=square},
  {black, mark=triangle},
  {black, mark=diamond}, 
  {black, mark=pentagon}, 
  {black, mark=*},
  {black, mark=square*},
  {black, mark=triangle*},
  {black, mark=diamond*}, 
  {black, mark=pentagon*}, 
}

\definecolor{darkgreen}{rgb}{0,0.4,0} 
\definecolor{darkbrown}{rgb}{0.5, 0.396, 0.09}

\definecolor{c1}{rgb}{0.0, 0.4196078431372549, 0.6431372549019608}
\definecolor{c2}{rgb}{1.0, 0.5019607843137255, 0.054901960784313725}
\definecolor{c3}{rgb}{0.6705882352941176, 0.6705882352941176,
0.6705882352941176} \definecolor{c}{rgb}{0.34901960784313724, 0.34901960784313724, 0.34901960784313724}
\definecolor{c4}{rgb}{0.37254901960784315, 0.6196078431372549,
0.8196078431372549} \definecolor{c}{rgb}{0.7843137254901961, 0.3215686274509804, 0.0}
\definecolor{c5}{rgb}{0.5372549019607843, 0.5372549019607843,
0.5372549019607843} \definecolor{c}{rgb}{0.6352941176470588, 0.7843137254901961, 0.9254901960784314}
\definecolor{c6}{rgb}{1.0, 0.7372549019607844, 0.4745098039215686}
\definecolor{c7}{rgb}{0.8117647058823529, 0.8117647058823529,
0.8117647058823529}

\pgfplotscreateplotcyclelist{myCycleListColor}
{%
  {blue, mark=o},
  {red, mark=square},
  {darkbrown, mark=triangle},
  {darkgreen, mark=diamond},
  {black, mark=pentagon},
  {blue, mark=*},
  {red, mark=square*},
  {darkbrown, mark=triangle*},
  {darkgreen, mark=diamond*},
  {black, mark=pentagon*},
}

% \pgfplotscreateplotcyclelist{myCycleListColor}
% {%
%   {c1, mark=o},
%   {c2, mark=square},
%   {c3, mark=triangle},
%   {c4, mark=diamond}, 
%   {c5, mark=pentagon}, 
%   {c1, mark=*},
%   {c2, mark=square*},
%   {c3, mark=triangle*},
%   {c4, mark=diamond*}, 
%   {c5, mark=pentagon*}, 
% }

\pgfplotsset{every axis/.append style= 
              {
                font=\small,
                mark size=2,
                line width = 0.1,
                %cycle list name=black white,
                legend style={font=\small, mark size=3, draw=none, fill=none},
                legend cell align=left,
                cycle list name=myCycleListColor,
              }
            }
            
\pgfplotstableset
{
  every odd row/.style={before row={\rowcolor[gray]{0.9}}},
  every head row/.style=
  {
    before row=
    {%
      \toprule
    },
    after row=\midrule
  },
  every last row/.style=
  {
    after row=\bottomrule
  }
}

% Boolean for drawing a bounding box around every figure or not.
\newif\ifdrawboundingbox

 
\usetikzlibrary{external} % Is activated with the command
\tikzset{external/system call={pdflatex \tikzexternalcheckshellescape
-halt-on-error -interaction=batchmode -jobname "\image" "\texsource"}} 
% '\tikzexternalize'.

%\tikzexternalize
% externalization.

\pgfkeys
{ 
  /pgf/number format/.cd,
  fixed,
  %fixed zerofill,
  set thousands separator={\,},
  1000 sep in fractionals,
}


==> general/titleAndAuthors.tex <==
\title{Smart octrees: Integration on trimmed patches in three dimensions}

 \author[1]{Laszlo Kudela \thanks{laszlo.kudela@tum.de, Corresponding Author}}
 \author[1]{some more authors\thanks{authors@tum.de}}
% \author[1]{Nils Zander\thanks{nils.zander@tum.de}}
% \author[1]{Tino Bog\thanks{tino.bog@tum.de}}
% \author[1]{Stefan Kollmannsberger}%\thanks{kollmannsberger@mytum.de}}
% \author[1]{Ernst Rank}%\thanks{ernst.rank@tum.de}}

\affil[1]{Chair for Computation in Engineering,
 Technische Universit\"at M\"unchen,
  Arcisstr. 21, 80333 M\"unchen, Germany}
 
\newcommand{\journal}{Some Fancy Journal}
\newcommand{\publicationDate}{\today}


==> sections/geometry.tex <==
\newpage
\section{Geometry Aquisition}
\subsection{Photogrammetry and Point Clouds}
\subsection{Assessing the Quality of Geometric Models}




